Modular Deep Active Learning Framework for Image Annotation: A Technical Report for the Ophthalmo-AI Project

Image annotation is one of the most essential tasks for guaranteeing proper treatment for patients and tracking progress over the course of therapy in the field of medical imaging and disease diagnosis. However, manually annotating a lot of 2D and 3D imaging data can be extremely tedious. Deep Learning (DL) based segmentation algorithms have completely transformed this process and made it possible to automate image segmentation. By accurately segmenting medical images, these algorithms can greatly minimize the time and effort necessary for manual annotation. Additionally, by incorporating Active Learning (AL) methods, these segmentation algorithms can perform far more effectively with a smaller amount of ground truth data. We introduce MedDeepCyleAL, an end-to-end framework implementing the complete AL cycle. It provides researchers with the flexibility to choose the type of deep learning model they wish to employ and includes an annotation tool that supports the classification and segmentation of medical images. The user-friendly interface allows for easy alteration of the AL and DL model settings through a configuration file, requiring no prior programming experience. While MedDeepCyleAL can be applied to any kind of image data, we have specifically applied it to ophthalmology data in this project.

==> old/old_backup.tex <==
% %% TEMPLATE TAKEN FROM https://www.overleaf.com/latex/templates/one-column-ieee-journal-article/ykctxqgxptrs




% %% bare_jrnl.tex
% %% V1.4b
% %% 2015/08/26
% %% by Michael Shell
% %% see http://www.michaelshell.org/
% %% for current contact information.
% %%
% %% This is a skeleton file demonstrating the use of IEEEtran.cls
% %% (requires IEEEtran.cls version 1.8b or later) with an IEEE
% %% journal paper.
% %%
% %% Support sites:
% %% http://www.michaelshell.org/tex/ieeetran/
% %% http://www.ctan.org/pkg/ieeetran
% %% and
% %% http://www.ieee.org/

% %%*************************************************************************
% %% Legal Notice:
% %% This code is offered as-is without any warranty either expressed or
% %% implied; without even the implied warranty of MERCHANTABILITY or
% %% FITNESS FOR A PARTICULAR PURPOSE! 
% %% User assumes all risk.
% %% In no event shall the IEEE or any contributor to this code be liable for
% %% any damages or losses, including, but not limited to, incidental,
% %% consequential, or any other damages, resulting from the use or misuse
% %% of any information contained here.
% %%
% %% All comments are the opinions of their respective authors and are not
% %% necessarily endorsed by the IEEE.
% %%
% %% This work is distributed under the LaTeX Project Public License (LPPL)
% %% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
% %% distributed and modified. A copy of the LPPL, version 1.3, is included
% %% in the base LaTeX documentation of all distributions of LaTeX released
% %% 2003/12/01 or later.
% %% Retain all contribution notices and credits.
% %% ** Modified files should be clearly indicated as such, including  **
% %% ** renaming them and changing author support contact information. **
% %%*************************************************************************


% % *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% % *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% % *** with production work. The IEEE's font choices and paper sizes can   ***
% % *** trigger bugs that do not appear when using other class files.       ***                          ***
% % The testflow support page is at:
% % http://www.michaelshell.org/tex/testflow/


% % Please refer to your journal's instructions for other
% % options that should be set.
% \documentclass[journal,onecolumn]{IEEEtran}
% %
% % If IEEEtran.cls has not been installed into the LaTeX system files,
% % manually specify the path to it like:
% % \documentclass[journal]{../sty/IEEEtran}

% % Some very useful LaTeX packages include:
% % (uncomment the ones you want to load)


% % *** MISC UTILITY PACKAGES ***
% %
% %\usepackage{ifpdf}
% % Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% % compilation based on whether the output is pdf or dvi.
% % usage:
% % \ifpdf
% %   % pdf code
% % \else
% %   % dvi code
% % \fi
% % The latest version of ifpdf.sty can be obtained from:
% % http://www.ctan.org/pkg/ifpdf
% % Also, note that IEEEtran.cls V1.7 and later provides a builtin
% % \ifCLASSINFOpdf conditional that works the same way.
% % When switching from latex to pdflatex and vice-versa, the compiler may
% % have to be run twice to clear warning/error messages.






% % *** CITATION PACKAGES ***
% %
% %\usepackage{cite}
% % cite.sty was written by Donald Arseneau
% % V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% % \cite{} output to follow that of the IEEE. Loading the cite package will
% % result in citation numbers being automatically sorted and properly
% % "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% % cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% % \cite will automatically add leading space, if needed. Use cite.sty's
% % noadjust option (cite.sty V3.8 and later) if you want to turn this off
% % such as if a citation ever needs to be enclosed in parenthesis.
% % cite.sty is already installed on most LaTeX systems. Be sure and use
% % version 5.0 (2009-03-20) and later if using hyperref.sty.
% % The latest version can be obtained at:
% % http://www.ctan.org/pkg/cite
% % The documentation is contained in the cite.sty file itself.

% % *** GRAPHICS RELATED PACKAGES ***
% %
% \ifCLASSINFOpdf
%   \usepackage[pdftex]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../pdf/}{../jpeg/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% \else
%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%   % will default to the driver specified in the system graphics.cfg if no
%   % driver is specified.
%   % \usepackage[dvips]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../eps/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.eps}
% \fi
% % graphicx was written by David Carlisle and Sebastian Rahtz. It is
% % required if you want graphics, photos, etc. graphicx.sty is already
% % installed on most LaTeX systems. The latest version and documentation
% % can be obtained at: 
% % http://www.ctan.org/pkg/graphicx
% % Another good source of documentation is "Using Imported Graphics in
% % LaTeX2e" by Keith Reckdahl which can be found at:
% % http://www.ctan.org/pkg/epslatex
% %
% % latex, and pdflatex in dvi mode, support graphics in encapsulated
% % postscript (.eps) format. pdflatex in pdf mode supports graphics
% % in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% % that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% % not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% % which can result in "jaggedy"/blurry rendering of lines and letters as
% % well as large increases in file sizes.
% %
% % You can find documentation about the pdfTeX application at:
% % http://www.tug.org/applications/pdftex

% % *** MATH PACKAGES ***
% %
% %\usepackage{amsmath}
% % A popular package from the American Mathematical Society that provides
% % many useful and powerful commands for dealing with mathematics.
% %
% % Note that the amsmath package sets \interdisplaylinepenalty to 10000
% % thus preventing page breaks from occurring within multiline equations. Use:
% %\interdisplaylinepenalty=2500
% % after loading amsmath to restore such page breaks as IEEEtran.cls normally
% % does. amsmath.sty is already installed on most LaTeX systems. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/amsmath

% % *** SPECIALIZED LIST PACKAGES ***
% %
% %\usepackage{algorithmic}
% % algorithmic.sty was written by Peter Williams and Rogerio Brito.
% % This package provides an algorithmic environment fo describing algorithms.
% % You can use the algorithmic environment in-text or within a figure
% % environment to provide for a floating algorithm. Do NOT use the algorithm
% % floating environment provided by algorithm.sty (by the same authors) or
% % algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% % algorithm float types and packages that provide these will not provide
% % correct IEEE style captions. The latest version and documentation of
% % algorithmic.sty can be obtained at:
% % http://www.ctan.org/pkg/algorithms
% % Also of interest may be the (relatively newer and more customizable)
% % algorithmicx.sty package by Szasz Janos:
% % http://www.ctan.org/pkg/algorithmicx

% % *** ALIGNMENT PACKAGES ***
% %
% %\usepackage{array}
% % Frank Mittelbach's and David Carlisle's array.sty patches and improves
% % the standard LaTeX2e array and tabular environments to provide better
% % appearance and additional user controls. As the default LaTeX2e table
% % generation code is lacking to the point of almost being broken with
% % respect to the quality of the end results, all users are strongly
% % advised to use an enhanced (at the very least that provided by array.sty)
% % set of table tools. array.sty is already installed on most systems. The
% % latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/array

% % IEEEtran contains the IEEEeqnarray family of commands that can be used to
% % generate multiline equations as well as matrices, tables, etc., of high
% % quality.

% % *** SUBFIGURE PACKAGES ***
% \ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
% \else
%  \usepackage[caption=false,font=footnotesize]{subfig}
% \fi




% % *** PDF, URL AND HYPERLINK PACKAGES ***
% %
% \usepackage{url}
% % url.sty was written by Donald Arseneau. It provides better support for
% % handling and breaking URLs. url.sty is already installed on most LaTeX
% % systems. The latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/url
% % Basically, \url{my_url_here}.




% % *** Do not adjust lengths that control margins, column widths, etc. ***
% % *** Do not use packages that alter fonts (such as pslatex).         ***
% % There should be no need to do such things with IEEEtran.cls V1.6 and later.
% % (Unless specifically asked to do so by the journal or conference you plan
% % to submit to, of course. )


% % correct bad hyphenation here
% % \hyphenation{op-tical net-works semi-conduc-tor}
% \usepackage{multicol}
% \usepackage{listings}
% \usepackage[numbers]{natbib}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{mdframed}
% \usepackage{titlesec}
% \usepackage{setspace}
% \onehalfspacing
% \titlespacing{\section}{12pc}{1.5ex plus .1ex minus .2ex}{1pc}
% \setcounter{secnumdepth}{3}

% \newcommand{\pyobject}[1]{\color{black}{\texttt{#1}}}



% % Define the new commands here

% \newenvironment{framedlisting}{\mdframed}{\endmdframed}
% \begin{document}
% %
% % paper title
% % Titles are generally capitalized except for words such as a, an, and, as,
% % at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% % not capitalized unless they are the first or last word of the title.
% % Linebreaks \\ can be used within to get better formatting as desired.
% % Do not put math or special symbols in the title.
% \title{Efficient image annotations in the Ophthalmo-AI project - Technical Report}
% %
% %
% % author names and IEEE memberships
% % note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% % a structure at a ~ so this keeps an author's name from being broken across
% % two lines.
% % use \thanks{} to gain access to the first footnote area
% % a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% % was not built to handle multiple paragraphs
% %

% \author{
% Md Abdul Kadir,
% Pascale Maul,
% Hans-Jürgen Profitlich, 
% Hasan Md Tusfiqur, 
% Moritz Wolf,
% Daniel Sonntag
% }

% % note the % following the last \IEEEmembership and also \thanks - 
% % these prevent an unwanted space from occurring between the last author name
% % and the end of the author line. i.e., if you had this:
% % 
% % \author{....lastname \thanks{...} \thanks{...} }
% %                     ^------------^------------^----Do not want these spaces!
% %
% % a space would be appended to the last name and could cause every name on that
% % line to be shifted left slightly. This is one of those "LaTeX things". For
% % instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% % "AB" then you have to do: "\textbf{A}\textbf{B}"
% % \thanks is no different in this regard, so shield the last } of each \thanks
% % that ends a line with a % and do not let a space in before the next \thanks.
% % Spaces after \IEEEmembership other than the last one are OK (and needed) as
% % you are supposed to have spaces between the names. For what it is worth,
% % this is a minor point as most people would not even notice if the said evil
% % space somehow managed to creep in.

% % The paper headers
% \markboth{}%
% {Kadir \MakeLowercase{\textit{et al.}}: Ophthalmo-AI Technical Report}
% % The only time the second header will appear is for the odd numbered pages
% % after the title page when using the twoside option.
% % 
% % *** Note that you probably will NOT want to include the author's ***
% % *** name in the headers of peer review papers.                   ***
% % You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% % you desire.

% % If you want to put a publisher's ID mark on the page you can do it like
% % this:
% %\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% % Remember, if you use this you must call \IEEEpubidadjcol in the second
% % column for its text to clear the IEEEpubid mark.

% % use for special paper notices
% %\IEEEspecialpapernotice{(Invited Paper)}

% % make the title area
% \maketitle

% % As a general rule, do not put math, special symbols or citations
% % in the abstract or keywords.
% \begin{abstract}
% Active learning (AL) algorithms have become increasingly popular for training models with limited data. However, selecting data for annotation remains challenging due to the limited information available on unseen data. 
% To address this issue, we present MedDeepCyleAL, an end-to-end framework implementing the complete active learning cycle, allowing researchers the flexibility of freely choosing the type of deep learning model they want to employ and which provides an annotation tool (AT) that supports not only classification but also the segmentation of medical images.
% The annotation tool provides all functionalities for area/line segmentation as well as labelling.
% MedDeepCyleAL is easy to use as the AL and DL model settings can be changed through a configuration file, requiring no prior programming experience of the user. 
% Our framework can be used for all types of pool-based AL applications.
% \end{abstract}

% % Note that keywords are not normally used for peerreview papers.
% % \begin{IEEEkeywords}
% % IEEE, IEEEtran, journal, \LaTeX, paper, template.
% % \end{IEEEkeywords}

% \section{Introduction}

% Optical Coherence Tomography (OCT) has been widely used in biomedical imaging. Ophthalmologists use the segmentation of ocular OCT images to diagnose,and treatment of eye diseases such as Diabetic Retinopathy (DR) and Diabetic Macular Edema (DME) \cite{dme}. 
% In recent years, Deep Learning (DL) based methods have achieved considerable success in medical image segmentation \cite{DL-MI}.
% However,their progress has often been constrained as they require large data set which are labeled by clinical expert.
% Labeling medical image data is a time-consuming and expensive process as domain experts are required to annotate them. 
% Active learning (AL) can be beneficial for medical image segmentation by reducing the burden of extensive annotation effort \cite{AL-MI}.

% % describe what AL is, describe AL iterative workflow

% % mention current AL trends, f.ex. check out this ACM survey paper (free access) DOI: https://doi.org/10.1145/3472291

% % define objectives of framework (see abstract & developping AL framework for medical imaging/ medical image segmentation) and write about our particular use case (OCT segmentation in ophthalmo AI)

% %talk about prior work, i.e. other AL framework that can, in contrast to our framework only be integrated programatically

% % list examples of active learning frameworks, check out this article: https://towardsdatascience.com/a-summary-of-active-learning-frameworks-3165159baae9

% % I think most prior frameworks did concentrate on classification (modAL) but rarely include segmentation cases segmentation, mention that for CV other frameworks do not provide an integrated AT, you would have to set up CVAT or similar yourself

% % talk about how we are using AL in ophthalmoAI f.ex. partial labelling and Abdul's pixel-based approach

% \begin{figure}[!h]
% \centering
% \includegraphics[width=2.5in]{imgs/ALCycle.jpg}
% \caption{
% Overview of the AL cycle and the functionality of the individual components.
% The first step consist of the annotation of an initial data set through the AT.
% The annotation information is then forwarded to a Controller, which initiates the update of the data set (2.) and triggers the next AL learning cycle (3.).
% The back-end then trains a deep learning model, and performs the querying of the non-annotated data (4.).
% The top $n$ samples, that result from the querying, are then send to the controller, which in turn sends the information to the AT (5.).
% With the help of a data preparation tool, the AT then downloads new samples (6.) and generates preliminary annotations with a pre-trained model. 
% Those preliminary annotations serve the purpose of facilitating the annotation process by proposing labels/ a segmentation, thus reducing annotation cost.
% The $n$ samples and their annotations are then reviewed by the oracle (1.).
% }
% \label{fig_sim}
% \end{figure}

% \subsection{The Ophthalmo-AI Project}
% The developments in the Ophthalmo-AI project are intended to support ophthalmologists with an intelligent assistance system in making a correct diagnosis based on image data and clinical data and in making the best possible therapy decision. For comprehensible suggestions for medical staff, the AI system will first label biological structures and pathological features in the image data. Then special AI models derive diagnoses from the image findings and other information from the patient file, make therapy suggestions and predict the success of the therapy. Interactive machine learning methods are used to integrate the doctors' knowledge of the case in question into the process.  A large volume of treatment data collected and processed on a special data integration platform is used for system development. The resulting augmented intelligence system will be tested in clinical demonstrators for its practical suitability for macular degeneration and diabetic retinopathy. 

% The project focuses on the two most common causes of blindness in people over fifty: age-related macular degeneration (AMD) and diabetic retinopathy (DR). AMD is caused by aging processes in the central retinal cells (macula = point of sharpest vision). Everyone has a buildup of waste products in this area throughout life, and some have irregular blood vessels growing from the choroid under the retina. They leak fluid and blood, causing symptoms of "distortions" and progressive vision loss ("wet" form of "late" AMD). Diabetic retinopathy can occur as a result of diabetes. Here, too, blood components can escape into the retinal tissue. From this, pathological new blood vessels – so-called “proliferations” – can grow on the retina. Heavy bleeding into the eye can occur from these very vulnerable vessels, which can cause retinal detachment. Retinopathy often leads to swelling (=edema) in the area of the macula, the so-called "diabetic macular edema", which can lead to visual disturbances.

% The layered representation of the retina, the "optical coherence tomography" (OCT), makes it possible to detect the finest changes and swellings such as the presence of irregular blood vessels in the area of the macula. This is important for the diagnosis and therapy monitoring of both diseases. New drugs are now available that suppress the growth of abnormal blood vessels and reduce swelling in the macula. These drugs are injected directly into the vitreous cavity of the eye (intravitreal drug delivery, IVOM). The IVOM must be repeated at different intervals, usually monthly, until vision has stabilized.

% In the first project phase, both textual annotations in the patient files and annotations of the retinal structures (especially layers and drusen) are made using specially developed tools. To optimize the required working time, a tool already supports the doctors with segmentation models and special graphic algorithms. To further reduce the time-consuming annotation process, so-called active learning algorithms are used, which specifically select those image data that promise the greatest benefit in the continuous improvement of the models. In a second step, the resulting neural networks serve to support diagnoses and therapy suggestions and predict the success of the therapy. In order to enable the doctors to understand the system decisions, in addition to the assessment of an existing disease, explanations of the results are also output in the form of interactive segmentation maps of the characteristics relevant to the diagnosis.

% In the following we describe the tools developed to support the mentioned first phase of collecting annotated data.

% \section{Objectives}


% \subsection{OCT Annotation}



% \section{Functionalities}

% \section{Architecture}
% \begin{figure}[!h]
% \centering
% \includegraphics[width=5in]{imgs/AL-infrastrucure.png}
% \caption{please describe this architecture, similar to the animated slide. The left part will be dropped later, this is only a placeholder}
% \end{figure}

% \subsection{System Component Description}


% \subsection{Controller}


% \subsection{Data-Manager}

% Data Manager is developed as an independent module to support the annotation tool and Machine learning backend architecture. A large volume of treatment data that are stored in \pyobject{XplOit}\footnote{https://ophthalmo-ai.fraunhofer.de} Data server are collected and processed in this module. The Controller module accesses the data manager, and its functionalities can be divided into three main parts. Securely downloading required patient treatment data from the server to the local development machine. Process the raw data, which are stored as a large Volume file, and extract unannotated OCT scan slices and other metadata, including patients' health records (EHRs), diagnosis, and treatments. Data-manager also contains functionalities to store and access the annotations provided by the Annotation Tool for OCT images. This module also provides APIs to access training/validation/test datasets which are accessed by Active Learning Backend via the controller module. Common APIs of Data-Manager class and their functionalities are briefly described below:

% \begin{itemize}
%     \item \pyobject{initialize(root\_dir:Path, database:DB)} : Initializing \pyobject{DataManager} class using the tables in database containing patient attributes. Required patient files stored in Volume format (\pyobject{.VOL}) are downloaded using \pyobject{Xploit} api. 
    
%     \item \pyobject{initialize\_with\_files(file\_path:Path) -> None} \pyobject{DataManager} class can also be initialized using this function, if the required files are already downloaded from the server and stored in the local system.
    
%     \item \pyobject{get\_unannotated\_set() -> List[Dict]} : Returns a list of dictionary containing the path of unannotated OCT images and associated meta data.
    
%     \item \pyobject{remove\_from\_unannotated\_set(file\_list:List[Dict]) -> None} : Removes object from the unannotated set when a batch of OCT slices are annotated.
    
%     \item \pyobject{update\_annotations(annotations:Dict[Dict]) -> None} : Given the annotation values from the Annotation Tool for an OCT image, this function produces the associated semantic masks and stores in a form of image file. 
    
%     \item \pyobject{get\_annotated\_set() -> List[Dict]} : Returns a list of dictionary containing the path annotated OCT images and their corresponding annotated masks. 
    
%     \item \pyobject{get\_dataloader(DATA\_ENUM:str) -> list[Dict]}: Returns the pre-processed dataset for machine learning model training. Input argument is a literal of three choices \pyobject{DATA\_ENUM=[`train',`validation',`test']}.
% \end{itemize}


% \subsection{Active-Learning Backend}
% \input{sections/al_backend}

% % analogous to AL iteration description in introduction describe one AL iteration but with our individual components

% % since we are using it for medical image segmentation, describe the unet and how we are using it
% \subsection{Annotation Tool}

% \section{Intelligent User Interfaces}

% \subsection{Annotation Tool}
% The annotation tool that is used for image annotations is a fork of HUMAN
% \cite{wolf-2020-human}. Its architecture was made to be compatible with Active Learning from the start with easy configurability and extensibility for new annotation tasks. To achieve this it employs a state machine, with 


% % web app, flask backend, sqlite database
% For efficient annotations of OCT images, a few changes were needed. For OCT annotations it is often necessary to jump back and forth between tasks. The 





% \subsection{Demos}

% \section{Discussion and Outlook}


% \bibliographystyle{IEEEtranN}
% \bibliography{references}

% \end{document}
